Learning and Composing Primitive Skills for Dual-arm Manipulation

In an attempt to confer robots with complex manipulation capabilities, dual-arm anthropomorphic systems have become an important research topic in the robotics community. Most approaches in the literature rely upon a great understanding of the dynamics underlying the system's behaviour and yet offer limited autonomous generalisation capabilities. To address these limitations, this work proposes a modelisation for dual-arm manipulators based on dynamic movement primitives laying in two orthogonal spaces. The modularity and learning capabilities of this model are leveraged to formulate a novel end-to-end learning-based framework which (i) learns a library of primitive skills from human demonstrations, and (ii) composes such knowledge simultaneously and sequentially to confront novel scenarios. The feasibility of the proposal is evaluated by teaching the iCub humanoid the basic skills to succeed on simulated dual-arm pick-and-place tasks. The results suggest the learning and generalisation capabilities of the proposed framework extend to autonomously conduct undemonstrated dual-arm manipulation tasks.

==> Sections/background.tex <==
\section{PRIMITIVE SKILLS as COUPLING TERMS} \label{sec:background}
    This paper pursues an end-to-end learning-based framework which endows a dual-arm system with enhanced generalisation capabilities, meets the synchronisation constraints, and is easily programmable and customisable by non-robotics-experts. In this work, all these requirements are addressed by means of learnable and composable primitive skills, which can be represented as \acfp{DMP}~\cite{ijspeert2013dynamical}. \acp{DMP} are a versatile tool for modelling and learning complex motions where: (a)~any movement can be efficiently learned and generated, (b)~a unique demonstration is already generalisable, (c)~convergence to the goal is guaranteed, and (d)~their representation is translation and time-invariant.
    
    A \ac{DMP} describes the dynamics of a primitive skill as a spring-damper system under the effect of a virtual external force called coupling term. A pure spring-damper system generates a continuous displacement between any initial and goal state. Any other dynamical behaviour, i.e. primitive skill, is explained by coupling terms. Importantly, these terms can be learnt from human demonstrations. Because of all these properties, \acp{DMP} are adapted to constitute the fundamental building blocks of this work. This section introduces the spring-damper system, which allows the encoding of any positional and orientational dynamics, and gives an overview of some of the coupling terms in the literature.

    % ===============================
    % ===============================
    % ===============================
    \subsection{Positional Dynamics}
        Let the current positional state of a one-\ac{DoF} system be defined by its position, linear velocity and acceleration. Then, the system's state transition is described by the following set of nonlinear differential equations:
        \begin{align}
            \tau \dot{z} &= \alpha_x (\beta_x (g_{x} - \pos) - z) + f{_{{x}}}(\boldsymbol{\cdot}), \label{eq:dmp_1} \\
            \tau \vel &= z, \label{eq:dmp_2}
        \end{align}
        where $\tau$ is a scaling factor for time, $\pos$ is the system's position, $z$ and $\dot{z}$ respectively are the scaled velocity and accelaration, $\alpha_x$ and $\beta_x$ are constants defining the positional system's dynamics, $g_{x}$ is the model's attractor, and ${f{_{{x}}}(\boldsymbol{\cdot})}$ is the coupling term. The coupling term applying at multiple \acp{DoF} at once is defined as $\adaptation{_{{x}}}$. The system will converge to $g_{x}$ with critically damped dynamics and null velocity when ${\tau > 0}$, ${\alpha_x > 0}$, $\beta_x > 0$ and ${\beta_x = \alpha_x / 4}$~\cite{ijspeert2013dynamical}.

    % ===============================
    % ===============================
    % ===============================
    \subsection{Orientational Dynamics}
        For rotations, it is important to choose a representation with no singularities and whose differentiation is numerically stable. However, there is no minimal definition of orientation lying in $\real^3$. One alternative uses rotation matrices ${\mathbf{R} \in \rotmat(3)}$ and individually describes the numerical change in each of the nine values of $\mathbf{R}$ as presented in~\eref{eq:dmp_1}-\eref{eq:dmp_2}. This method, however, does not guarantee that the orthogonality requirements for rotation matrices are met at all times.

        Another possible representation is the unit quaternions ${\vq \in \real^4 = \sphere^3}$~\cite{ude2014orientation}. They address the assumption of independence between numerical values by encoding the rotation as a whole, at the cost of more computationally expensive calculations. Let the current orientational state of a system be defined by its orientation, angular velocity and acceleration. Then, the orientational state transition is described by the following nonlinear differential equations:
        \begin{align}
           \tau \bm{\dot{\eta}} &= \alpha_q (\beta_q \; 2 \log (\vgoal_{q} \ast \bar{\vq}) - \bm{\eta}) + \adaptation{_{{q}}}, \label{eq:q_dmp_1} \\
           \tau \vdq &= \frac{1}{2} \bm{\eta} \ast \vq, \label{eq:q_dmp_2}
        \end{align}
        where $\vq$ is the system's orientation, $\bm{\eta}$ and $\bm{\dot{\eta}}$ respectively are the scaled angular velocity and acceleration, $\alpha_q$ and $\beta_q$ are constants defining the system's dynamics, $\vgoal_{q} \in \sphere^3$ is the model's attractor, and ${\adaptation{_{{q}}} \in \real^4}$ is the coupling term. The operators $\log(\cdot)$, $\ast$, and $\bar{\vq}$ denote the logarithm, multiplication and conjugate operations for quaternions, respectively.

    % ===============================
    % ===============================
    % ===============================
    \subsection{Coupling Terms}
        Coupling terms describe the system's behaviour, thus being useful to learn and retrieve any primitive skill. They are commonly used to encode the positional~\cite{ijspeert2013dynamical} and orientational~\cite{ude2014orientation} dynamics of a motion. Coupling terms are modelled in each dimension as a weighted linear combination of non-linear \acp{RBF} distributed along the trajectory. Thus, learning a certain movement relies on finding the weights of the \acp{RBF} which closely reproduce a demonstrated skill. 
        
        More complex behaviours may be achieved by exploiting an additional coupling term simultaneously with the motion-encoding one. This approach has been used to avoid joint limits and constraining the robot's workspace via repulsive forces pushing the system away from these limits~\cite{gams2009line}. Coupling terms have also been leveraged for obstacle avoidance with an analytic biologically-inspired approach describing how humans steer around obstacles~\cite{hoffmann2009biologically,rai2014learning}. Another use is for environmental and self-interaction purposes by means of a controller tracking a desired force profile~\cite{gams2014coupling}. To the best of the authors' knowledge, the practice of using coupling terms simultaneously has been limited to two primitive skills acting on the same frame or space~\cite{pastor2009learning}. Contrarily, this work further exploits the \ac{DMP} modularity to describe a dual-arm system in two orthogonal spaces with the purpose of facing complex scenarios by composing multiple coupling terms.

==> Sections/extension.tex <==
%\section{DUAL-ARM DYNAMIC MOVEMENT PRIMITIVES} \label{sec:extension}
\section{DUAL-ARM SYSTEM MODELISATION} \label{sec:extension}
    To jointly deal with the trajectory planning and environmental interaction requirements, while meeting the dual-arm synchronisation constraints, this work expands the previously presented \ac{DMP}-based modelisation to the dual-arm context. The proposed approach considers the representation of any possible dual-arm primitive skill in two different spaces. This allows the manipulator to exploit the dynamic system formulation to learn and execute different actions in both spaces. This section firstly introduces the proposed typology of actions, and then describes the corresponding model of the dual-arm system and its grasping.

    % ===============================
    % ===============================
    % ===============================
    \subsection{Dual-arm Primitive Skills Taxonomy} \label{sec:formulation_taxonomy}
        Skills for single-arm manipulation have been well analysed in the robotics community. While some of this knowledge can be extrapolated for a dual-arm manipulator as a whole, their complexity resides in the arms interaction. In the context of manipulation via a dual-arm system, a possible classification of any primitive skill falls into two groups: (a)~absolute skills, which imply a change of configuration of the manipulated object in the Cartesian or absolute space $\Askill$, e.g. move or turn an object in a particular manner, and (b)~relative skills, which exert an action on the manipulated object in the object or relative space $\Rskill$, e.g. opening a bottle's screw cap, or hold a parcel employing force contact.

        Each type of primitive skill uniquely produces movement in its space since they lay in orthogonal spaces such that $\Askill \perp \Rskill$. It is natural to expect from a dual-arm system to simultaneously carry out, at least, one absolute and one relative skill to accomplish a task. Let us analyse the task of moving a bottle to a particular position while opening its screw cap. Both end-effectors synchronously move to reach the desired configuration (absolute skill). At the same time, the left end-effector is constrained to hold the bottle upright (relative skill), while the right end-effector unscrews the cap (relative skill).

    % ===============================
    % ===============================
    % ===============================
    \subsection{Dual-arm DMP-based Modelisation}
        Given the variety of primitive skills that a dual-arm system can execute, this work seeks to model the robotic platform in a generalisable yet modular fashion, which accounts for both absolute and relative skills. To this aim, let us consider the closed kinematic chain depicted in \fref{fig:system} operating in a \ac{3D} workspace ${\workspace = \real^3 \times \rotmat(3)}$. Each arm $i$, where $i=\{L,\;R\}$, interacts with the same object $\object$. In this context, the absolute skill explains the movement of the object $\object$ in the workspace $\workspace = \Askill$, while the relative skill describes the actions of each end-effector $i$ in $\Rskill$, i.e. with respect to the object's reference frame $\{\object\}$. Note that $\{\object\}$ is the centre of the closed-chain dual-arm system.

        \begin{figure}[t!]
            \centering
            \includegraphics[width=5cm]{./Figures/da}
            \caption{\ac{DMP}-based modelisation of a closed-chain dual-arm system in the absolute and relative spaces~\cite{pairet2018learning}. This model is extended to deal with rotational dynamics.}
            \label{fig:system}
        \end{figure}

        The state of the closed-chain dual-arm system in the workspace can be described by the position/orientation, linear/angular velocities and accelerations of $\{\object\}$ in $\Askill$. The system's state transition is subjected to its dynamics. \fref{fig:system} illustrates the proposed modelisation of the system's dynamics in $\Askill$ as a set of \acp{DMP} acting between the objects's frame $\{\object\}$ and its goal configuration $\vgoal_o$, which accounts for a desired goal position $\vgoal_{o_x} \in \real^3$ and orientation $\vgoal_{o_q} \in \real^4$. Therefore, three positional \acp{DMP} as in \eref{eq:dmp_1}-\eref{eq:dmp_2} and one orientational \ac{DMP} as in \eref{eq:q_dmp_1}-\eref{eq:q_dmp_2} are required to encode the system's dynamics in the absolute space ${\Askill = \real^3 \times \rotmat(3)}$. In the relative space $\Rskill$, the dynamics of each end-effector are modelled as \acp{DMP} with respect to the objects's \mbox{frame $\{\object\}$}. Since ${\Rskill = \real^3 \times \rotmat(3)}$, each end-effector dynamic's in the relative frame is described by three positional \acp{DMP} as in \eref{eq:dmp_1}-\eref{eq:dmp_2} and one orientational \ac{DMP} as in \eref{eq:q_dmp_1}-\eref{eq:q_dmp_2}. 
        
        Any action referenced to the object's frame can be projected to the end-effectors using the grasping geometry $\graspmatrix$ of the manipulated object. This allows computing the required end-effector control commands to achieve a particular absolute task. A detailed explanation of this transformation can be found in~\cite{pairet2018learning}.
        
    % % ===============================
    % % ===============================
    % % ===============================
    % \subsection{Dual-arm Grasping Geometry}
    %     Any action referenced to the object's frame can be projected to the end-effectors using the grasping geometry of the manipulated object. This allows computing the required end-effector control commands to achieve a particular absolute task. For the end-effector $i$ there is a mapping or grasping matrix $\graspmatrix_i$ which establishes a velocity relation between the contact point $C_i$ and the system's frame $\{\object\}$ as:
    %     \begin{align}
    %         \vdy_{C_i} &= \graspmatrix_i^T \; \vdy_o,
    %     \end{align}
    %     where, for a workspace ${\workspace = \real^3 \times \rotmat(3)}$, ${\vdy_{C_i} \in \real^6}$ and ${\vdy_o \in \real^6}$ are the concatenation of the positional velocity ${\vvel \in \real^3}$ and Euler angular velocity $Euler(\vdq) \in \real^3$ of the contact point $C_i$ and the system's frame $\{\object\}$, respectively.
        
    %     The grasping matrix of the end-effector $i$ is defined as:
    %     \begin{align}
    %         \graspmatrix_i \in \real^{6 \times 6} =
    %         \begin{bmatrix}
    %             \mathbf{I}_{3 \times 3} & \mathbf{O}_{3 \times 3} \\
    %             \mathbb{S}(\vr_i) & \mathbf{I}_{3 \times 3}
    %             \label{eq:grasp_matrix}
    %         \end{bmatrix},
    %     \end{align}
    %     where $\mathbf{I}_{3 \times 3}$ is the identity matrix, and $\mathbb{S}(\vr_i) \in \real^{3 \times 3}$ is the skew-symmetric matrix performing the cross product:
    %     \begin{align}
    %         \mathbb{S}(\vr_i) =
    %         \begin{bmatrix}
    %             0 & -r_z & r_y \\
    %             r_z & 0 & -r_x \\
    %             -r_y & r_x & 0
    %         \end{bmatrix},
    %         \label{eq:skew_matrix}
    %     \end{align}
    %     where $\vr_i$ is the distance from the object's reference frame $\{\object\}$ to the contact point $C_i$.

    %     A global grasp map $\graspmatrix$ for the dual-arm manipulator can be defined by horizontally concatenating the grasp matrix of each end-effector, i.e. ${\graspmatrix = [\graspmatrix_L \; \graspmatrix_R] \in \real^{6 \times 12}}$ where $\graspmatrix_L$ and $\graspmatrix_R$ are the left and right arm grasp matrix, respectively.

